A survey on algorithmic aspects of modular decomposition

The modular decomposition is a technique that applies but is not restricted to graphs. The notion of module naturally appears in the proofs of many graph theoretical theorems. Computing the modular decomposition tree is an important preprocessing step to solve a large number of combinatorial optimization problems. Since the first polynomial time algorithm in the early 70's, the algorithmic of the modular decomposition has known an important development. This paper survey the ideas and techniques that arose from this line of research.

==> md-survey-arxiv.bbl.tex <==
\newcommand{\etalchar}[1]{$^{#1}$}
\begin{thebibliography}{BXHLdM09}

\bibitem[AA05]{AA05}
M.~Albert and M.~Atkinson.
\newblock Simple permutations and pattern restricted permutations.
\newblock {\em Discrete Mathematics}, 300(1-3):1 -- 15, 2005.

\bibitem[AS02]{AS02}
M.~Atkinson and T.~Stitt.
\newblock Restricted permutations and the wreath product.
\newblock {\em Discrete Mathematics}, 259(1-3):19 -- 36, 2002.

\bibitem[BBCP04]{BBCP05}
A.~Bergeron, S.~B\'erard, C.~Chauve, and C.~Paul.
\newblock Sorting by reversal is not always difficult.
\newblock In {\em Workshop on Algorithm for Bio-Informatics (WABI)}, Lecture
  Notes in Computer Science, 2004.

\bibitem[BBCP07]{BBCP07}
S.~B{\'e}rard, A.~Bergeron, C.~Chauve, and C.~Paul.
\newblock Perfect sorting by reversals is not always difficult.
\newblock {\em IEEE/ACM Trans. Comput. Biology Bioinform.}, 4(1):4--16, 2007.

\bibitem[BBT08]{BBT08}
S.~B{\"o}cker, Q.B.~Anh Bui, and A.~Tru{\ss}.
\newblock An improved fixed-parameter algorithm for minimum-flip consensus
  trees.
\newblock In {\em International Workshop on Parameterized and Exact Computation
  (IWPEC)}, number 5018 in Lecture Notes in Computer Science, pages 43--54,
  2008.

\bibitem[BCdMR05]{BCMR05}
A.~Bergeron, C.~Chauve, F.~de~Montgolfier, and M.~Raffinot.
\newblock Computing common intervals of $k$ permutations, with applications to
  modular decomposition of graphs.
\newblock In {\em European Symposium on Algorithms (ESA)}, number 3669 in
  Lecture Notes in Computer Science, pages 779--790, 2005.

\bibitem[BCdMR08]{BCMR08}
Anne Bergeron, Cedric Chauve, Fabien de~Montgolfier, and Mathieu Raffinot.
\newblock Computing common intervals of k permutations, with applications to
  modular decomposition of graphs.
\newblock {\em SIAM Journal on Discrete Mathematics}, 22(3):1022--1039, 2008.

\bibitem[BCHP03]{BCHP03}
A.~Bretscher, D.G. Corneil, M.~Habib, and C.~Paul.
\newblock A simple linear time {L}ex{BFS} cograph recognition algorithm.
\newblock In {\em 29th International Workshop on Graph-Theoretic Concepts in
  Computer Science (WG)}, volume 2880 of {\em Lecture Notes in Computer
  Science}, pages 119--130, 2003.

\bibitem[BCHP08]{BCHP08}
A.~Bretscher, D.~Corneil, M.~Habib, and C.~Paul.
\newblock A simple linear time lexbfs cograph recognition algorithm.
\newblock {\em SIAM Journal on Discrete Mathematics}, 22(4):1277--1296, 2008.

\bibitem[BCP08]{BCP08}
S.~B{\'e}rard, C.~Chauve, and C.~Paul.
\newblock A more efficient algorithm for perfect sorting by reversals.
\newblock {\em Information Processing Letters}, 106:90--95, 2008.

\bibitem[BFG{\etalchar{+}}09]{BFG09}
St{\'e}phane Bessy, Fedor~V. Fomin, Serge Gaspers, Christophe Paul, Anthony
  Perez, Saket Saurabh, and St{\'e}phan Thomass{\'e}.
\newblock Kernels for feedback arc set in tournaments.
\newblock Technical Report CoRR abs/0907.2165, arxiv, 2009.

\bibitem[BHS02]{BHS02}
A.~Bergeron, S.~Herber, and J.~Stoye.
\newblock Common intervals and sorting by reversals: a mariage of necessity.
\newblock In {\em European Conference on Computational Biology},
  Bioinformatics, pages 54--63, 2002.

\bibitem[Bla78]{Bla78}
A.~Blass.
\newblock Graphs with unique maximal clumpings.
\newblock {\em Journal of Graph Theory}, 2:19--24, 1978.

\bibitem[BLS99]{BLS99}
A.~Brandst{\"a}dt, VB. Le, and J.~Spinrad.
\newblock {\em Graph classes: a survey}.
\newblock SIAM Monographs on Discrete Mathematics and Applications. Society for
  Industrial and Applied Mathematics, 1999.

\bibitem[BPP09]{BPP09}
S.~Bessy, C.~Paul, and A.~Perez.
\newblock Polynomial kernels for 3-leaf power graph modification problems.
\newblock In {\em International Workshop on Combinatorial Algorithm (IWOCA)},
  Lecture Notes in Computer Science, 2009.

\bibitem[BR06]{BR06}
M.~Bouvel and D.~Rossin.
\newblock The longest common pattern problem for two permutations.
\newblock {\em Pure Mathematics and Applications}, 17(1-2):55--69, 2006.

\bibitem[BRV07]{BRV07}
M.~Bouvel, D.~Rossin, and S.~Vialette.
\newblock Longest common separable pattern among permutations.
\newblock In {\em Annual Symposium on Combinatorial Pattern Matching (CPM)},
  number 4580 in Lecture Notes in Computer Science, pages 316--327, 2007.

\bibitem[BX08]{Bui08}
B.M. Bui-Xuan.
\newblock {\em Tree-representation of set families in graph decompositions and
  efficient algorithms}.
\newblock PhD thesis, Univ. de Montpellier II, 2008.

\bibitem[BXH08]{BH08}
B.-M. Bui-Xuan and M.~Habib.
\newblock A representation theorem for union-difference families and
  application.
\newblock In {\em Latin American Symposium on Theoretical Informatics (LATIN)},
  volume 4957 of {\em Lecture Notes in Computer Science}, pages 492--503, 2008.

\bibitem[BXHLdM09]{BHLM09}
B-M. Bui-Xuan, M.~Habib, V.~Limouzy, and F.~de~Montgolfier.
\newblock Algorithmic aspects of a general modular decomposition theory.
\newblock {\em Discrete Applied Mathematics}, 157(9):1993--2009, 2009.

\bibitem[BXHP05]{BHP05}
B.-M. Bui-Xuan, M.~Habib, and C.~Paul.
\newblock Revisiting uno and yagiura's algorithm.
\newblock In {\em 16th International Symposium on Algorithms and Computation
  (ISAAC)}, volume 3827 of {\em Lecture Notes in Computer Science}, pages
  146--155, 2005.

\bibitem[Cai96]{Cai96}
L.~Cai.
\newblock Fixed-parameter tractability of graph modification problems for
  hereditary properties.
\newblock {\em Information Processing Letters}, 58(4):171--176, 1996.

\bibitem[Cap97]{Cap97}
C.~Capelle.
\newblock {\em D\'ecomposition de graphes et permutations factorisantes}.
\newblock PhD thesis, Univ. de Montpellier II, 1997.

\bibitem[CE80]{CE80}
W.H. Cunnigham and J.~Edmonds.
\newblock A combinatorial decomposition theory.
\newblock {\em Canadian Journal of Mathematics}, 32(3):734--765, 1980.

\bibitem[CER93]{CER93}
B.~Courcelle, J.~Engelfriet, and G.~Rozenberg.
\newblock Handle rewriting graph grammars.
\newblock {\em Journal of Computer and System Science}, 46:218--270, 1993.

\bibitem[CH94]{CH94}
A.~Cournier and M.~Habib.
\newblock A new linear algorithm of modular decomposition.
\newblock In {\em Trees in algebra and programming (CAAP)}, volume 787 of {\em
  Lecture Notes in Computer Science}, pages 68--84, 1994.

\bibitem[CH97]{CH97}
C.~Capelle and M.~Habib.
\newblock Graph decompositions and factorizing permutations.
\newblock In {\em Fifth Israel Symposium on Theory of Computing and Systems -
  ISTCS, IEEE Conf. PR08037, Ramat-Gan, Israel}, pages 132--143, 1997.

\bibitem[CHdM02]{CHM02}
C.~Capelle, M.~Habib, and F.~de~Montgolfier.
\newblock Graph decompositions and factorizing permutations.
\newblock {\em Discrete Mathematics and Theoretical Computer Science},
  5:55--70, 2002.

\bibitem[CHM81]{CHM81}
M.~Chein, M.~Habib, and M.-C. Maurer.
\newblock Partitive hypergraphs.
\newblock {\em Discrete Mathematics}, 37:35--50, 1981.

\bibitem[CI98]{CI98}
A.~Cournier and P.~Ille.
\newblock Minimal indecomposable graphs.
\newblock {\em Discrete Mathematics}, 183:61--80, 1998.

\bibitem[CJS72]{CJS72}
D.D. Cowan, L.O. James, and R.G. Stanton.
\newblock Graph decomposition for undirected graphs.
\newblock In {\em 3rd S-E Conference on Combinatorics, Graph Theory and
  Computing, Utilitas Math}, pages 281--290, 1972.

\bibitem[CLR90]{CLR90}
T.H. Cormen, C.E. Leiserson, and R.L. Rivest.
\newblock {\em Algorithms}.
\newblock MIT Press, 1990.

\bibitem[CLSB81]{CLS81}
D.G. Corneil, H.~Lerchs, and L.K. Stewart-Burlingham.
\newblock Complement reducible graphs.
\newblock {\em Discrete Applied Mathematics}, 3(1):163--174, 1981.

\bibitem[Cor04a]{Cor04b}
D.~G. Corneil.
\newblock A simple 3-sweep {LBFS} algorithm for the recognition of unit
  interval graphs.
\newblock {\em Discrete Applied Mathematics}, 138(3):371--379, 2004.

\bibitem[Cor04b]{Cor04}
D.G. Corneil.
\newblock Lexicographic {B}readth {F}irst {S}earch - a survey.
\newblock In {\em 30th International Workshop on Graph-Theoretic Concepts in
  Computer Science (WG)}, volume 3353 of {\em Lecture Notes in Computer
  Science}, pages 1--19, 2004.

\bibitem[CP06]{CP06}
C.~Crespelle and C.~Paul.
\newblock Fully-dynamic recognition algorithm and certificate for directed
  cographs.
\newblock {\em Discrete Applied Mathematics}, 154(12):1722--1741, 2006.

\bibitem[CPS85]{CPS85}
D.G. Corneil, Y.~Perl, and L.K. Stewart.
\newblock A linear time recognition algorithm for cographs.
\newblock {\em SIAM Journal on Computing}, 14(4):926--934, 1985.

\bibitem[Cre09]{Cre09}
C.~Crespelle.
\newblock Fully dynamic representation of interval graphs.
\newblock In {\em Internation Workshop on Graph Theoretical Concepts in
  Computer Science (WG)}, 2009.

\bibitem[Cun82]{Cun82}
W.H. Cunningham.
\newblock Decomposition of directed graphs.
\newblock {\em SIAM Journal on Algebraic and Discrete Methods}, 3:214--228,
  1982.

\bibitem[Dah95]{Dah95}
E.~Dahlhaus.
\newblock Efficient parallel algorithms for cographs and distance hereditary
  graphs.
\newblock {\em Discrete Applied Mathematics}, 57:29--54, 1995.

\bibitem[DF99]{DF99}
R.G. Downey and M.R. Fellows.
\newblock {\em Parameterized complexity}.
\newblock Springer, 1999.

\bibitem[DGH{\etalchar{+}}06]{DGH06b}
M.~Dom, J.~Guo, F.~H{\"u}ffner, R.~Niedermeier, and A.~Truss.
\newblock Fixed-parameter tractability results for feedback set problems in
  tournaments.
\newblock In {\em Italian Conference on Algorithms and Complexity (CIAC)},
  volume 3998 of {\em Lecture Notes in Computer Science}, pages 320--331, 2006.

\bibitem[DGM01]{DGM01}
E.~Dahlhaus, J.~Gustedt, and R.M. McConnell.
\newblock Efficient and practical algorithm for sequential modular
  decomposition algorithm.
\newblock {\em Journal of Algorithms}, 41(2):360--387, 2001.

\bibitem[dM03]{Mon03}
F.~de~Mongolfier.
\newblock {\em D\'ecomposition modulaire des graphes - Th\'eorie, extensions et
  algorithmes}.
\newblock PhD thesis, Univ. de Montpellier II, 2003.

\bibitem[EG97]{EG77}
J.~Edmonds and R.~Giles.
\newblock A min-max relation for submodular functions on graphs.
\newblock {\em Annals of Discrete Mathematics}, 1:185--204, 1997.

\bibitem[EGMS94]{EGMS94}
A.~Ehrenfeucht, H.N. Gabow, R.M. McConnell, and S.L. Sullivan.
\newblock An {$O(n^2)$} divide-and-conquer algorithm for the prime tree
  decomposition of two-structures and modular decomposition of graphs.
\newblock {\em Journal of Algorithms}, 16:283--294, 1994.

\bibitem[EHR99]{EHR99}
A.~Ehrenfeucht, T.~Harju, and G.~Rozenberg.
\newblock {\em The theory of 2-structures}.
\newblock World Scientific, 1999.

\bibitem[ER90]{ER90}
A.~Ehrenfeucht and G.~Rozenberg.
\newblock Primitivity is hereditary for 2-structures.
\newblock {\em Theoretical Computer Science}, 70(3):343 -- 358, 1990.

\bibitem[FG06]{FG06}
J.~Flum and M.~Grohe.
\newblock {\em Parameterized complexity theorey}.
\newblock Texts in Theoretical Computer Science. Springer, 2006.

\bibitem[FHdMV04]{FHMV04}
J.-L. Fouquet, M.~Habib, F.~de~Montgolfier, and J.-M. Vanherpe.
\newblock Bimodular decomposition of bipartite graphs.
\newblock In {\em International Workshop on Graph Theoretical Concepts in
  Computer Science (WG)}, volume 3353 of {\em Lecture Notes in Computer
  Science}, pages 117--128, 2004.

\bibitem[FLRS07]{FLR07}
M.R. Fellows, M.~Langston, F.~Rosamond, and P.~Shaw.
\newblock Efficient parameterized preprocessing for cluster editing.
\newblock In {\em International Symposium on Fundamentals of Computation Theory
  (FCT)}, number 4639 in Lecture Notes in Computer Science, pages 312--321,
  2007.

\bibitem[FP03]{FP03}
Jir\'{\i} Fiala and Dani{\"e}l Paulusma.
\newblock The computational complexity of the role assignment problem.
\newblock In {\em International Colloquium on Automata, Languages and
  Programming (ICALP)}, volume 2719 of {\em Lecture Notes in Computer Science},
  pages 817--828, 2003.

\bibitem[Gal67]{Gal67}
T.~Gallai.
\newblock Transitiv orientierbare graphen.
\newblock {\em Acta Mathematica Acad. Sci. Hungar.}, 18:25--66, 1967.

\bibitem[GHKZ08]{GHKZ08}
J.~Guo, F.~H{\"u}ffner, C.~Komusiewicz, and Y.~Zhang.
\newblock Improved algorithms for bicluster editing.
\newblock In {\em Annual Conference on Theory and Applications of Models of
  Computation (TAMC)}, volume 4978 of {\em Lecture Notes in Computer Science},
  pages 445--456, 2008.

\bibitem[Gol80]{Gol80}
M.C. Golumbic.
\newblock {\em Algorithmic graph theory and perfect graphs}.
\newblock Academic Press, 1980.

\bibitem[GP07]{GP07}
E.~Gioan and C.~Paul.
\newblock Dynamic distance hereditary graphs using split decomposition.
\newblock In {\em International Symposium on Algorithms and Computation
  (ISAAC)}, volume 4884 of {\em Lecture Notes in Computer Science}, 2007.

\bibitem[GPTC09a]{GPTC09b}
E.~Gioan, C.~Paul, M.~Tedder, and D.~Corneil.
\newblock Practical split-decomposition via graph-labelled trees.
\newblock Submitted, 2009.

\bibitem[GPTC09b]{GPTC09a}
E.~Gioan, C.~Paul, M.~Tedder, and D.~Corneil.
\newblock Quasi-linear circle graph recognition.
\newblock Submitted, 2009.

\bibitem[Guo07]{Guo07}
J.~Guo.
\newblock A more effective linear kernelization for cluster editing.
\newblock In {\em International SymposiumCombinatorics, Algorithms,
  Probabilistic and Experimental Methodologies (ESCAPE)}, volume 4614 of {\em
  Lecture Notes in Computer Science}, pages 36--47, 2007.

\bibitem[HdMP04]{HMP04}
M.~Habib, F.~de~Montgolfier, and C.~Paul.
\newblock A simple linear-time modular decomposition algorithm.
\newblock In {\em 9th Scandinavian Workshop on Algorithm Theory (SWAT)}, volume
  3111 of {\em Lecture Notes in Computer Science}, pages 187--198, 2004.

\bibitem[HHS95]{HHS95}
M.~Habib, M.~Huchard, and J.S. Spinrad.
\newblock A linear algorithm to decompose inheritance graphs into modules.
\newblock {\em Algorithmica}, 13:573--591, 1995.

\bibitem[HM79]{HM79}
M.~Habib and M.-C. Maurer.
\newblock On the $x$-join decomposition of undirected graphs.
\newblock {\em Discrete Applied Mathematics}, 1:201--207, 1979.

\bibitem[HM91]{HM91}
W.-L. Hsu and T.-H. Ma.
\newblock Substitution decomposition on chordal graphs and applications.
\newblock In {\em 2nd International Symposium on Algorithms (ISA)}, volume 557
  of {\em Lecture Notes in Computer Science}, pages 52--60, 1991.

\bibitem[HMPV00]{HMPV00}
M.~Habib, R.M. McConnell, C.~Paul, and L.~Viennot.
\newblock Lex-bfs and partition refinement, with applications to transitive
  orientation, interval graph recognition and consecutive ones testing.
\newblock {\em Theoretical Computer Science}, 234:59--84, 2000.

\bibitem[HMS09]{HMS09}
S.~Herber, R.~Mayr, and J.~Stoye.
\newblock Common intervals of multiple permutations.
\newblock {\em Algorithmica}, 2009.

\bibitem[Hop71]{Hop71}
J.~Hopcroft.
\newblock An $n\log n$ algorithm for minimizing states in a finite automaton.
\newblock {\em Theory of machines and computations}, pages 189--196, 1971.

\bibitem[HP05]{HP05}
M.~Habib and C.~Paul.
\newblock A simple linear time algorithm for cograph recognition.
\newblock {\em Discrete Applied Mathematics}, 145(2):183--187, 2005.

\bibitem[HPV98]{HPV98}
M.~Habib, C.~Paul, and L.~Viennot.
\newblock A synthesis on partition refinement: a useful routine for strings,
  graphs, boolean matrices and automata.
\newblock In {\em 15th Symposium on Theoretical Aspect of Computer Science
  (STACS)}, volume 1373 of {\em Lecture Notes in Computer Science}, pages
  25--38, 1998.

\bibitem[HPV99]{HPV99}
M.~Habib, C.~Paul, and L.~Viennot.
\newblock Partition refinement : an interesting algorithmic tool kit.
\newblock {\em International Journal of Foundation of Computer Science},
  10(2):147--170, 1999.

\bibitem[HSS01]{HSS01}
P.~Hell, R.~Shamir, and R.~Sharan.
\newblock A fully dynamic algorithm for recongizing and representing propoer
  interval graphs.
\newblock {\em SIAM Journal on Discrete Mathematics}, 31(1):289--305, 2001.

\bibitem[Hsu92]{Hsu92}
W.-L. Hsu.
\newblock A simple test for interval graphs.
\newblock In {\em 3rd International Symposium on Algorithms and Computation
  (ISAAC)}, volume 557 of {\em Lecture Notes in Computer Science}, pages
  459--468, 1992.

\bibitem[Iba09]{Iba09}
L.~Ibarra.
\newblock A fully dynamic graph algorithm for recognizing interval graphs.
\newblock {\em Algorithmica}, 2009.

\bibitem[JO92a]{JO92}
B.~Jamison and S.~Olariu.
\newblock Recognizing $p_4$-sparse graphs in linear time.
\newblock {\em SIAM Journal on Discrete Mathematics}, 21:381--406, 1992.

\bibitem[JO92b]{JO92b}
B.~Jamison and S.~Olariu.
\newblock A tree representation of $p_4$-sparse graphs.
\newblock {\em Discrete Applied Mathematics}, 35:115--129, 1992.

\bibitem[JO95]{JO95}
B.~Jamison and S.~Olariu.
\newblock P-components and the homogeneous decomposition of graphs.
\newblock {\em SIAM Journal on Discrete Mathematics}, 8(3):448--463, 1995.

\bibitem[Lov72]{Lov72}
L.~Lov\'asz.
\newblock A characterization of perfect graphs.
\newblock {\em Journal of Combinatorial Theory Series B}, 13:95--98, 1972.

\bibitem[M{\"o}h85a]{Moh85b}
R.H. M{\"o}hring.
\newblock Algorithmic aspect of comparability graphs and interval graphs.
\newblock {\em Graphs and orders}, pages 42--101, 1985.

\bibitem[M{\"o}h85b]{Moh85}
R.H. M{\"o}hring.
\newblock Algorithmic aspect of the substitution decomposition in optimization
  over relations, set systems and boolean functions.
\newblock {\em Annals of Operations Research}, 4:195--225, 1985.

\bibitem[MR84]{MR84}
R.H. M{\"o}hring and F.J. Radermacher.
\newblock Substitution decomposition for discrete structures and connections
  with combinatorial optimization.
\newblock {\em Annals of Discrete Mathematics}, 19:257--356, 1984.

\bibitem[MS89]{MS89}
J.H. Muller and J.P. Spinrad.
\newblock Incremental modular decomposition.
\newblock {\em Journal of the ACM}, 36(1):1--19, 1989.

\bibitem[MS94]{MS94}
R.M. McConnell and J.P. Spinrad.
\newblock Linear-time modular decomposition and efficient transitive
  orientation of comparability graphs.
\newblock In {\em 5th Annual ACM-SIAM Symposium on Discrete Algorithms (SODA)},
  pages 536--545, 1994.

\bibitem[MS99]{MS99}
R.M. McConnell and J.P. Spinrad.
\newblock Modular decomposition and transitive orientation.
\newblock {\em Discrete Mathematics}, 201:189--241, 1999.

\bibitem[MS00]{MS00}
R.M. McConnell and J.P. Spinrad.
\newblock Ordered vertex partitioning.
\newblock {\em Discrete Mathematics and Theoretical Computer Science},
  4:45--60, 2000.

\bibitem[Nie06]{Nie06}
R.~Niedermeier.
\newblock {\em Invitation to fixed parameter algorithms}, volume~31 of {\em
  Oxford Lectures Series in Mathematics and its Applications}.
\newblock Oxford University Press, 2006.

\bibitem[PdSS07]{PSS07}
F.~Protti, M.~Dantas da~Silva, and J.L. Szwarcfiter.
\newblock Applying modular decomposition to parameterized cluster editing
  problems.
\newblock {\em Theory of Computing Systems}, 2007.

\bibitem[PT87]{PT87}
R.~Paigue and R.E. Tarjan.
\newblock Three partition refinement algorithms.
\newblock {\em SIAM Journal on Computing}, 16(6):973--989, 1987.

\bibitem[RST08]{RST08}
I.~Rapaport, K.~Suchan, and I.~Todinca.
\newblock Minimal proper interval completions.
\newblock {\em Information Processing Letters}, 106(5):195--202, 2008.

\bibitem[RTL76]{RTL76}
D.J. Rose, R.E. Tarjan, and G.S. Lueker.
\newblock Algorithmic aspects of vertex elimination on graphs.
\newblock {\em SIAM Journal on Computing}, 5(2):266--283, 1976.

\bibitem[Spi03]{Spi03}
J.P. Spinrad.
\newblock {\em Efficient graph representation}, volume~19 of {\em Fields
  Institute Monographs}.
\newblock American Mathematical Society, 2003.

\bibitem[SS04]{SS04}
R.~Shamir and R.~Sharan.
\newblock A fully dynamic algorithm for modular decomposition and recognition
  of cographs.
\newblock {\em Discrete Applied Mathematics}, 136(2-3):329--340, 2004.

\bibitem[ST93]{ST93b}
J.~Schmerl and W.~Trotter.
\newblock Critically indecomposable partially ordered sets, graphs, tournaments
  and other binary relational structures.
\newblock {\em Discrete Mathematics}, 113(1-3):191 -- 205, 1993.

\bibitem[Sum73]{Sum73}
D.P. Sumner.
\newblock Graphs indecomposable with respect to the $x$-join.
\newblock {\em Discrete Mathematics}, 6:281--298, 1973.

\bibitem[TCHP08]{TCHP08}
M.~Tedder, D.~Corneil, M.~Habib, and C.~Paul.
\newblock Simpler linear-time modular decomposition via recursive factorizing
  permutations.
\newblock In {\em International Colloquium on Automata, Languages and
  Programming (ICALP)}, volume 5125 (1) of {\em Lecture Notes in Computer
  Science}, pages 634--645, 2008.

\bibitem[UY00]{UY00}
T.~Uno and M.~Yagiura.
\newblock Fast algorithms to enumerate all common intervals of two
  permutations.
\newblock {\em Algorithmica}, 26(2):290--309, 2000.

\end{thebibliography}

